Throughput Maximizing Takeoff Scheduling for eVTOL Vehicles in On-Demand Urban Air Mobility Systems

Urban Air Mobility (UAM) offers a solution to current traffic congestion by using electric Vertical Takeoff and Landing (eVTOL) vehicles to provide on-demand air mobility in urban areas. Effective traffic management is crucial for efficient operation of UAM systems, especially for high-demand scenarios. In this paper, we present a centralized framework for conflict-free takeoff scheduling of eVTOLs in on-demand UAM systems. Specifically, we provide a scheduling policy, called VertiSync, which jointly schedules UAM vehicles for servicing trip requests and rebalancing, subject to safety margins and energy requirements. We characterize the system-level throughput of VertiSync, which determines the demand threshold at which the average waiting time transitions from being stable to being increasing over time. We show that the proposed policy maximizes throughput for sufficiently large fleet size and if the UAM network has a certain symmetry property. We demonstrate the performance of VertiSync through a case study for the city of Los Angeles, and show that it significantly reduces average passenger waiting time compared to a first-come first-serve scheduling policy.

==> TODO.tex <==
\section{\textcolor{red}{To DO}}\label{section:ToDo}
\begin{enumerate}
    \item \textcolor{red}{Expand on the literature of UAM traffic management in the introduction.}
    \item \textcolor{red}{Reference code on Github.}
\end{enumerate}




==> proof-renewal-sufficient-2.tex <==
\section{Proof of Theorem \ref{thm:renewal-sufficient-2}}\label{section:proof-renewal-sufficient-2}
We follow the same line of proof as in Theorem~\ref{thm:renewal-sufficient}. For brevity, we only highlight the major differences.

At the start of the $(k+1)$-th cycle, we solve the LP \eqref{eq:linear-program} and we let $K_{i}^{*}$, $i \in [\numsafesch]$, be its solution. We then construct a feasible solution to the optimization problem \eqref{eq:TFMP-objective}-\eqref{eq:TFMP-energy-constraints} as follows:
\begin{enumerate} 
\item Choose a service vector $\routingvec{}{i} \in \safeschset$ with $K_{i}^{*} > 0$, and, before activating $\routingvec{}{i}$, distribute the aircraft in the system so that for any $p \in \routeset$ with $\routingvec{p}{i} > 0$, there is
    \begin{equation*}
       \aircraftcard_p := \frac{\routingvec{p}{i}}{\sum_{p \in \routeset}\routingvec{p}{i}}\aircraftcard 
    \end{equation*}
    aircraft at vertiport $o_p$. The initial distribution of aircraft takes at most $\aircraftcard \overline{T}$ minutes.
\item Once the initial distribution is completed and the airspace is empty, activate $\routingvec{}{i}$ for a duration of 
\begin{equation*}
    \max_{p \in \routeset: \routingvec{p}{i} > 0} \frac{\aircraftcard_p}{\routingvec{p}{i}}\cruisetau
\end{equation*}
minutes. At the end of this interval, $\aircraftcard_p$ trips (out of $\Queuelength{p}(t_{k+1})$) will be serviced for all $p \in \routeset$. 
\item Once step 2 is completed and the airspace is empty, we re-balance the aircraft using $\routingvec{}{i}$'s ``reversed" service vector, i.e., a service vector $\routingvec{}{j} \in \safeschset$ such that for all $p \in \routeset$ with $\routingvec{p}{i} > 0$, $\routingvec{q}{j} = \routingvec{p}{i}$, where $q = (d_p,o_p)$ is the opposite O-D pair to the pair $p$. It takes at most $\overline{T}$ minutes for the airspace to become empty, and an additional $\lceil E_{p}/E_{\text{inc}}\rceil \cruisetau$ recharging time before the first aircraft is ready for rebalancing. Therefore, the rebalancing process takes at most
\begin{equation*}
        \max_{p \in \routeset: \routingvec{p}{i} > 0} \left(\frac{\aircraftcard_p}{\routingvec{p}{i}} + \lceil\frac{E_{p}}{E_{\text{inc}}}\rceil \right)\cruisetau + \overline{T}
\end{equation*} 
minutes. 
\item Repeat steps 1 to 3 until the service vector is used for a total duration of $(K_{i}^{*}+1)\cruisetau$ minutes. This will take at most 
\begin{equation*}
    N_p := \left\lceil \frac{\routingvec{p}{i} K_i^{*}}{\aircraftcard_p} \right\rceil + \left\lfloor \frac{\routingvec{p}{i} K_i^{*}}{\aircraftcard_p} \right\rfloor 
\end{equation*}
number of iterations. Therefore, steps 1 to 3 are repeated for a total duration of  
\begin{equation*}
     \max_{p \in \routeset: \routingvec{p}{i} > 0} (\left(\frac{\aircraftcard_p}{\routingvec{p}{i}} + \lceil\frac{E_{p}}{E_{\text{inc}}}\rceil \right)\cruisetau + \overline{T})N_p
\end{equation*}
minutes. At the end of this time interval, $\routingvec{p}{i} K_i^{*}$ trips will be serviced for all $p \in \routeset$.
\item Repeat steps 1 to 3 for another service vector in $\safeschset$. Once these steps are completed for every service vector $\routingvec{}{i} \in \safeschset$ with $K_{i}^{*} > 0$, $\sum_{i=1}^{\numsafesch}\routingvec{p}{i}K_{i}^{*}$ requests will be serviced for each O-D pair $p \in \routeset$. From the constraint of the LP \eqref{eq:linear-program}, it follows that all the requests for the $(k+1)$-th cycle will be serviced and the cycle ends.
\end{enumerate}
By combining all the above steps, it follows that
\begin{equation}\label{eq:cycle-upper-bound-2}
\begin{aligned}
        \Cyclelength(k+1) &\leq \sum_{i=1}^{\numsafesch}\max_{p \in \routeset: \routingvec{p}{i} > 0} (\left(\frac{\aircraftcard_p}{\routingvec{p}{i}} + \lceil\frac{E_{p}}{E_{\text{inc}}}\rceil \right)\cruisetau + \overline{T})N_p \\
        &\leq C_1 \sum_{i=1}^{\numsafesch} K_i^{*} + C_2,
\end{aligned}
\end{equation}
where 
\begin{equation*}
    \begin{aligned}
        C_1 &= 2 + \frac{2}{\aircraftcard}\max_{i}\left( \frac{\overline{T}}{\cruisetau} + \max_{p \in \routeset: \routingvec{p}{i} > 0}\lceil \frac{E_p}{E_{\text{inc}
        }} \rceil  \right)\sum_{p \in \routeset}\routingvec{p}{i} \\
        C_2 &= \frac{\overline{T}}{\cruisetau}\numsafesch + \sum_{i = 1}^{\numsafesch} \left(\frac{\aircraftcard}{\sum_{p \in \routeset}\routingvec{p}{i}} + \max_{p \in \routeset: \routingvec{p}{i} > 0} \lceil \frac{E_p}{E_{\text{inc}}} \rceil \right).
    \end{aligned}
\end{equation*}
\par
Similar to the proof of Theorem~\ref{thm:renewal-sufficient}, we can cast the network as an irreducible, aperiodic discrete-time Markov chain with the state $\{\Queuelength{}(t_k)\}_{k \geq 1}$. By letting $\Cyclelength(k)=n$, it follows that, with probability one, $\lim_{n \ra \infty}\Queuelength{p}(t_{k+1})/n = \Arrivalrate{p}$. Since $\Arrivalrate{} \in D_{1}^{\circ}$, with probability one, there exists non-negative $x_1, x_2, \ldots, x_{\numsafesch}$ with $\sum_{i=1}^{\numsafesch}x_i < 1$ such that $\Queuelength{}(t_{k+1})/n < \sum_{i=1}^{\numsafesch}\routingvec{}{i}x_i/C_1$. For $i \in [\numsafesch]$, define $K_i := nx_i/C_1$. Then, $K_i$'s are a feasible solution to the LP \eqref{eq:linear-program}, and $\sum_{i=1}^{\numsafesch}K_i < n/C_1$. This, combined with \eqref{eq:cycle-upper-bound-2}, implies that, with probability one,
\begin{equation*}
    \limsup_{n \ra \infty}\left(\frac{\Cyclelength(k+1)}{n}\right)^2 < 1.
\end{equation*}
The rest of the proof is the same as the prof of Theorem~\ref{thm:renewal-sufficient}.

